A Two-Stage Progressive Pre-training using Multi-Modal Contrastive Masked Autoencoders

In this paper, we propose a new progressive pre-training method for image understanding tasks which leverages RGB-D datasets. The method utilizes Multi-Modal Contrastive Masked Autoencoder and Denoising techniques. Our proposed approach consists of two stages. In the first stage, we pre-train the model using contrastive learning to learn cross-modal representations. In the second stage, we further pre-train the model using masked autoencoding and denoising/noise prediction used in diffusion models. Masked autoencoding focuses on reconstructing the missing patches in the input modality using local spatial correlations, while denoising learns high frequency components of the input data. Moreover, it incorporates global distillation in the second stage by leveraging the knowledge acquired in stage one. Our approach is scalable, robust and suitable for pre-training RGB-D datasets. Extensive experiments on multiple datasets such as ScanNet, NYUv2 and SUN RGB-D show the efficacy and superior performance of our approach. Specifically, we show an improvement of +1.3% mIoU against Mask3D on ScanNet semantic segmentation. We further demonstrate the effectiveness of our approach in low-data regime by evaluating it for semantic segmentation task against the state-of-the-art methods.

==> 0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> ablation/curriculum.tex <==
\begin{table}[h!]
\centering

%\resizebox{0.80\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline

\hline

\hline
Curriculum order  &  mIoU \\
\hline

\hline

\hline


Contrastive $\rightarrow$ MIM + denoising + global distill  & \textbf{67.5} \\ \hline

MIM + denoising $\rightarrow$ Contrastive & 64.9 \\ \hline

Contrastive + MIM + denoising & 64.2 \\ \hline

\end{tabular}
%}%
\caption {\label{tab:ablation_curriculum} Effect of ordering of pre-training strategies on ScanNet 2D semantic segmentation.}
\end{table}

==> ablation/initialization.tex <==
\begin{table}[h!]

\centering

%\resizebox{0.80\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline

\hline

\hline
Method  & Backbone  & mIoU \\
\hline

\hline

\hline

Train from Scratch & ViT-B & 32.6\\ \hline

Mask3D~\cite{mask3d} & ViT-B & 41.3\\ \hline

Ours & ViT-B & \textbf{42.1} \\ \hline


\end{tabular}
%}%
\vspace{5pt}
\caption {\label{tab:ablation_init} Without ImageNet initialization, our approach still outperforms Mask3D.}
\end{table}

==> ablation/new_ablation.tex <==
\begin{table*}[h]
  %\tablestyle{4pt}{1}
  
  \begin{minipage}{0.5\linewidth}
  %\small
  \tablestyle{4pt}{1.05}
  %\renewcommand{\arraystretch}{0.3}
  \begin{tabular}{c|c}
    \hline
    
    \hline
    
    \hline
    Curriculum order  &  mIoU \\
    \hline
    
    \hline
    
    \hline
    
    Contrastive $\rightarrow$ MIM + denoising  & \textbf{67.0} \\ \hline
    
    MIM + denoising $\rightarrow$ Contrastive & 64.9 \\ \hline
    
    Contrastive + MIM + denoising & 64.2 \\ \hline
    
    \end{tabular}
    %}%
    \vspace{5pt}
    \caption {\small \label{tab:ablation_curriculum} Effect of ordering of pre-training strategies on \textbf{ScanNet 2D semantic segmentation}.}
  \end{minipage}
  
  %\hspace{10.0\linewidth}
  %\hfill
  \hspace{27em}
  %\small
  %\hfill
  \begin{minipage}{0.5\linewidth}
  \vspace{-8em}
  \tablestyle{4pt}{1.05}
  %\small
  %\renewcommand{\arraystretch}{0.3}
    \begin{tabular}{c|c|c}
    \hline
    
    \hline
    
    \hline
    Loss  & Backbone  & mIoU \\
    \hline
    
    \hline
    
    \hline
    
    MIM + Denoising & ViT-B & 66.3\\ \hline
    
    Depth + RGB Reconstruction & ViT-B & 66.4 \\ \hline
    
    Full & ViT-B & \textbf{67.0} \\ \hline
    
    \end{tabular}
    %}%
    \vspace{5pt}
    \caption {\small \label{tab:ablation_loss} Ablation study of different loss functions on \textbf{ScanNet 2D semantic segmentation}.}

  %\vspace{-20pt}
  \end{minipage}%\hspace{-1.0\textwidth}

  %\hfill
  %\vspace{-20em}
  \begin{minipage}{0.4\linewidth}
  %\flushleft
  %\vspace{-8em}
  \tablestyle{4pt}{1.05}
  %\centering
  %\renewcommand{\arraystretch}{0.3}
  \begin{tabular}{c|c|c}
    \hline
    
    \hline
    
    \hline
    Method  & Backbone  & mIoU \\
    \hline
    
    \hline
    
    \hline
    
    w/out noise & ViT-B & 66.2 \\ \hline
    
    noise only  & ViT-B & 66.7 \\ \hline
    
    Full & ViT-B & \textbf{67.0} \\ \hline
    
    
   \end{tabular}
    %}%
   \vspace{5pt}
   \caption {\small \label{tab:ablation_denoising} Ablation study on the components of the denoising method. We report the performance on \textbf{ScanNet 2D semantic segmentation}.}

  %\vspace{-20pt}
  \end{minipage}%\hspace{-1.0\textwidth}

  %\hfill
  \hspace{27em}
  %\renewcommand{\arraystretch}{0.3}
  \begin{minipage}{0.5\linewidth}
  \vspace{-10em}
  \tablestyle{4pt}{1.05}
  \begin{tabular}{c|c|c}
    \hline
    
    \hline
    
    \hline
    RGB ratio  & Depth ratio  & mIoU \\
    \hline
    
    \hline
    
    \hline
    
    20.0\% & 20.0\% & 65.2\\ \hline
    
    20.0\% & 50.0\% & 64.9\\ \hline
    
    20.0\% & 80.0\% & 65.0\\ \hline
    
    50.0\% & 20.0\% & 65.5\\ \hline
    
    50.0\% & 50.0\% & 65.1\\ \hline
    
    80.0\% & 20.0\% & 65.7\\ \hline
    
    80.0\% & 80.0\% & \textbf{67.0} \\ \hline
    
    
    \end{tabular}
    %}%
    \vspace{5pt}
    \caption {\label{tab:ablation_masking} Effect of different masking ratios for RGB and depth modality on \textbf{ScanNet 2D semantic segmentation}.}
    \end{minipage}

%\vspace{-20pt}
\end{table*}

==> ade_segt.tex <==
\begin{table*}[h!]
\centering

\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\hline

\hline

\hline
Methods  & Reconstruction task  & Backbone &  Pre-train  & Fine-tune Modality  & mIoU \\
\hline

\hline

\hline


MAE~\cite{mae}  & RGB                                                                      & ViT-B    &  ImageNet& RGB        & 46.2  \\ \hline


Mask3D~\cite{mask3d}   & Depth                                                                       & ViT-B    & ImageNet + ScanNet     & RGB        & 45.8 \\ \hline

MultiMAE*~\cite{multimae}  & RGB + Depth                                                                       & ViT-B    & ImageNet+ScanNet & RGB       &  45.9 \\ \hline


\textbf{Ours}  & Depth & ViT-B    & ImageNet+ScanNet   & RGB        & -  \\
\hline

\hline

\hline

MultiMAE~\cite{multimae}  & RGB + Depth + Segmentation                                                                     & ViT-B    & ImageNet & RGB       &  46.2 \\

\hline

\hline

\hline
\end{tabular}
}%
\caption {\label{tab:ade} \textbf{ADE-20k Semantic Segmentation}. }
\end{table*}
